The landscape of ontologies in materials science and engineering: A survey and evaluation

Ontologies are widely used in materials science to describe experiments, processes, material properties, and experimental and computational workflows. Numerous online platforms are available for accessing and sharing ontologies in Materials Science and Engineering (MSE). Additionally, several surveys of these ontologies have been conducted. However, these studies often lack comprehensive analysis and quality control metrics. This paper provides an overview of ontologies used in Materials Science and Engineering to assist domain experts in selecting the most suitable ontology for a given purpose. Sixty selected ontologies are analyzed and compared based on the requirements outlined in this paper. Statistical data on ontology reuse and key metrics are also presented. The evaluation results provide valuable insights into the strengths and weaknesses of the investigated MSE ontologies. This enables domain experts to select suitable ontologies and to incorporate relevant terms from existing resources.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/Conclusion_outlook_0.tex <==
\section{Conclusion and Outlook}
\label{sec:Conclusion_outlook}

In summary, the goal of this study is to improve knowledge representation in the field of Materials Science and  Engineering by identifying relevant ontologies and helping domain experts to choose the most appropriate ones for their specific requirements. These ontologies have multiple benefits: they enable us to recognize existing ontology design patterns, identify mappings between different ontologies, and find the Top-level ontologies used in the field.

As part of our future work, we intend to focus on identifying and extracting Ontology Design Patterns from MSE domain ontologies \cite{valentina_odp_extraction}. This process will involve collaborating with domain experts to ensure the effective utilization of these patterns in the development of ontologies. By doing so, we aim to enhance the quality and re-usability of ontologies within the domain of Materials Science and Engineering.

%\textcolor{blue}{
%\begin{itemize}
%    \item Which ontology can you recommend based on your results? 
%\end{itemize}
%}

% Outlook: 
    % Which ontologies are there?
    % Which ontology design patterns exist?
    % Which mappings exist between ontologies?
    % Which Top-level ontologies are used

%annotate the identified ontologies using the standard vocabularies, such as Vocabulary of Interlinked Datasets (VoID)\footnote{\url{http://vocab.deri.ie/void}} and Metadata for Ontology Description and publication (MOD)\footnote{\url{https://w3id.org/mod/2.0}}. Moreover, we will evaluate and assess the ontologies based on the FAIR data principles~\cite{wilkinson2016fair}.%, utilizing the available metrics, such as O’FAIRe~\cite{ofaire}, to determine the degree of FAIRness.

==> sections/introduction_0.tex <==
\section{Introduction}
\label{sec:intro}

The field of Materials Science and Engineering (MSE) has seen a rapid increase in the number of available ontologies, taxonomies, terminologies, and vocabularies to semantically describe various aspects of research, such as experimental procedures, material properties, computational workflows, and experimental outcomes~\cite{zhangoverview}. Some online repositories and portals offer access to these MSE ontologies including MatPortal\footnote{\url{https://matportal.org/}}, BioPortal\footnote{\url{https://bioportal.bioontology.org/}}, and IndustryPortal\footnote{\url{http://industryportal.enit.fr/}} among others. However, a major drawback is the limited number of ontologies registered and published in these ontology portals. In addition, the metadata information provided for ontologies in many repositories is often insufficient, which hinders the understanding of the ontology's scope and domain, making it challenging for MSE domain experts to assess its relevance to their specific requirements. Only two surveys, \cite{zhangoverview} and \cite{bernd_overview_2022}, have been published on ontologies in the MSE domain. However, it is important to note that these surveys lack comprehensive evaluations and quality assessments of the ontologies they cover. The survey conducted by Zhang et al. \cite{zhangoverview} evaluates nine ontologies, but six of these ontologies are not currently available online, which limits the accessibility and verification of their contents.
- Add other survey, add the drawbacks of other surveys

As a result, MSE domain experts find it challenging to identify and select the appropriate ontologies for their intended applications. Therefore, to support MSE domain experts in selecting the appropriate ontologies, a comprehensive review of ontologies, taking into account all the existing ontologies and including information regarding ontology reuse in the MSE domain, is necessary. The intention of this paper is to provide such a review and analysis to enable MSE domain experts to choose the appropriate ontologies. In particular, this study aims at answering to the following objectives:

\begin{itemize}
\item Investigating how to support domain experts to be able to select the ontologies they want to use, this involves: %\textcolor{blue}{This is not a question. Suggestion: Which criteria are relevant for a domain expert to choose a particular ontology? Which information about a MSE ontology does a domain expert need for selecting an ontology? Which information is relevant for a domain expert to make a proper choice of an MSE ontology to work with? }
    \begin{itemize}
        \item The identification of currently available ontologies in the domain of MSE.
        \item Understanding the specific purposes that these ontologies serve.
        %\item RQ1.c: How are ontologies used to represent the domain knowledge? \textcolor{blue}{This is not clear for me.}
    \end{itemize}


\item Exploring the ontology evaluation criteria that are relevant for a domain expert when selecting an ontology for use in MSE
%\textcolor{blue}{ RQ2.a What are the ontology evaluation criteria that can be carried out? RQ2.b Which ones are relevant for a domain expert and why?}
\end{itemize}

The paper is structured as follows: Section \ref{sec:method} describes the methodology used to collect and evaluate the MSE ontologies. In Section \ref{sec:results_discussion}, we present the quantitative results of the review process, as well as a thorough discussion of these findings in the context of our study objectives. Section \ref{sec:Conclusion_outlook} summarizes the primary outcomes of this study and outlines potential future research.


==> sections/method_0.tex <==
\section{Methodology}
\label{sec:method}

The methodology used in this paper combines expert knowledge with a systematic search of ontologies registered by various portals. The presented work was initiated by analyzing the results of an internal survey that was conducted in the Platform Material Digital (PMD) project\footnote{\url{https://www.materialdigital.de/}}. The PMD project involves industry-led pilot projects who share the common requirement of (re)using ontologies in the MSE domain. For this study, 13 projects were interviewed to gather essential information about the ontologies utilized in the field of Materials Science and Engineering. Additionally, ontology reference publications and overview papers ~\cite{zhangoverview, bernd_overview_2022, Andre_Bernd_2023, bwmd_review} were used to complete the list of ontologies. The ontologies selected for this review are required to meet specific criteria such as being relevant to disciplines of materials science and being used in related projects. A total of 41 ontologies have been identified, which are shared on GitHub\footnote{\href{https://github.com/ebrahimnorouzi/mseo.github.io}{Link to the GitHub repository including the list of ontologies and evaluation results}}.

For collecting metadata related to a specific ontology, an online search was conducted on the ontology homepage or ontology repository. The following criteria were used to analyze and assess the identified ontologies:

\begin{itemize}
\item[$\bullet$] \textbf{General Aspects of an Ontology:}
\begin{itemize}
\item \textbf{Name of the Ontology:} The full name.
\item \textbf{Acronym:} A shortened form.
\item \textbf{License:} Type of license (e.g., CC BY 4.0, MIT).
\item \textbf{Preferred Namespace:} The designated namespace for terms.
\item \textbf{Ontology Description:} A brief summary.
\item \textbf{Ontology Category:} Classification based on domain and scope.
\item \textbf{Ontology Accessibility:} Access information (e.g., URL, repository).
\end{itemize}

\item[$\bullet$] \textbf{Coverage of an Ontology:}
\begin{itemize}
\item \textbf{Domain:} Specific field or discipline (e.g., materials science, crystallography).
\item \textbf{Purpose:} Intended use or application (e.g., representing experimental data).
\end{itemize}

\item[$\bullet$] \textbf{Usage of an Ontology:}
\begin{itemize}
\item \textbf{Projects that Use the Ontology:} Notable projects or initiatives.
\item \textbf{Reference Papers:} Academic papers referencing the ontology.
\item \textbf{Citations:} Number and context of citations.
\item \textbf{Ontologies that Reuse an Ontology:} Other ontologies incorporating it.
\end{itemize}

\item[$\bullet$] \textbf{Ontology Design Information:}
\begin{itemize}
\item \textbf{Syntax:} Formal language used (e.g., OWL, RDF).
\item \textbf{Competency Questions:} Questions demonstrating its capability.
\item \textbf{Logical Expressivity:} Extent and complexity of logical constructs.
\item \textbf{Usage of Ontology Design Patterns:} Utilization of design patterns.
\item \textbf{Ontology Engineering Methodology:} Development process and principles.
\end{itemize}
\end{itemize}

\section*{Ontology Evaluation Metrics}

For the ontology evaluation, the following detailed metrics were examined:

\begin{itemize}
\item \textbf{Attribute Richness:} Measures the diversity of attributes used. \textit{Higher values indicate more knowledge conveyed. This is important because it reflects the level of detail and the ability of the ontology to represent complex information.}

\item \textbf{Inheritance Richness:} Indicates the extent of subclass relationships. \textit{Low values suggest a vertical structure, while high values suggest a horizontal structure. This is important as it shows how well knowledge is categorized and structured within the ontology.}

\item \textbf{Relationship Richness:} Assesses the variety and complexity of relationships defined in the ontology. \textit{Higher values indicate more information. This is crucial for understanding the interconnectedness of concepts within the ontology.}

\item \textbf{Axiom Class Ratio:} Ratio of axioms to classes, indicating logical assertion density. \textit{Low values suggest poor axiomatisation; extremely high values suggest over axiomatisation. This is significant as it shows the level of detail in logical definitions and constraints within the ontology.}

\item \textbf{Equivalence Ratio:} Proportion of equivalence axioms, reflecting similarity between classes. \textit{This metric helps in understanding the degree of redundancy and synonymy within the ontology.}

\item \textbf{Class/Property Ratio:} Describes the ratio between classes and relations. \textit{Low values indicate many properties connecting few concepts; high values indicate many concepts connected by few properties. This is important for evaluating the balance between concepts and their interrelationships.}

\item \textbf{Absolute Root Cardinality (NoR):} Number of root classes. \textit{Indicates cohesion; interpretation depends on the total number of classes. This metric is important for understanding the foundational structure of the ontology.}

\item \textbf{Absolute Leaf Cardinality (NoL):} Number of leaf classes. \textit{Indicates cohesion; interpretation depends on the total number of classes. This metric is crucial for assessing the granularity and detail of the ontology.}

\item \textbf{Absolute Depth:} Depth from root to leaf nodes. \textit{This metric shows the hierarchical complexity of the ontology, which is important for understanding the depth of the ontology's structure.}

\item \textbf{Average Depth (ADIT-LN):} Average depth of the ontology hierarchy. \textit{Indicates cohesion; interpretation depends on the ontology size. This metric helps in assessing the overall hierarchical organization.}

\item \textbf{Maximal Depth:} Maximum depth of the ontology hierarchy. \textit{This metric provides insights into the longest path from root to leaf, showing the extent of the deepest subcategories.}

\item \textbf{Absolute Breadth:} Breadth at each level of the ontology. \textit{This metric indicates the number of sibling classes at different levels, reflecting the ontology's width.}

\item \textbf{Average Breadth:} Average breadth across levels. \textit{Indicates horizontal modeling; should be interpreted relative to the number of classes. This metric helps in understanding the balance between depth and breadth in the ontology.}

\item \textbf{Maximal Breadth:} Maximum breadth across levels. \textit{This metric shows the widest part of the ontology, providing insights into the most extensive level of categorization.}

\item \textbf{Tangledness:} Degree of interconnectivity within the ontology. \textit{Values range from 0 (no tangledness) to 1 (high tangledness). This metric is important for evaluating the complexity and overlap in the hierarchical structure.}
\end{itemize}

These criteria and metrics provide a comprehensive evaluation framework for assessing the quality, usability, and effectiveness of ontologies in the domain of Materials Science and Engineering.

\begin{table}[h!]
\centering
\caption{Quality requirements and their justifications with mapped criteria}
\begin{tabular}{|m{6cm}|>{\centering\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{2.6cm}|}
\hline
\textbf{Quality Requirements} & \textbf{Justification} & \textbf{Mapped Criteria} \\
\hline
REQ1: The ontology must provide a comprehensive taxonomy covering necessary sub-domains of materials science. & The term "comprehensive" suggests that the ontology should be complete and cover all necessary sub-domains. & Completeness, Coverage, Availability \\
\hline
REQ2: The ontology should be capable of representing both experimental and simulation data. & The capability to represent various types of data indicates a complete and adaptable ontology. & Completeness, Adaptability, Availability \\
\hline
REQ3: The ontology should accurately represent relations between different concepts. & Accuracy is crucial for representing relationships, and relevancy ensures that these relationships matter to the domain. & Accuracy, Relevancy, Availability \\
\hline
REQ4: The ontology must standardize and unify metadata descriptions in compliance with existing standards. & Standardization implies compliance and internal consistency. & Compliance, Internal Consistency, Availability \\
\hline
REQ5: The ontology must provide comprehensive representations for experimental settings, outcomes, high-throughput analysis data, and literature. & Comprehensive representations imply completeness and coverage. & Completeness, Coverage, Availability \\
\hline
REQ6: The ontology must facilitate trustworthy and verifiable quality management of data. & Trustworthiness and verifiability imply credibility and accuracy. & Credibility, Accuracy, Availability \\
\hline
REQ7: The ontology should enable querying specifically designed for machine learning model development. & Specificity for machine learning makes it relevant and complex and comprehensive for that purpose. & Relevancy, Complexity, Comprehensibility, Availability \\
\hline
REQ8: The ontology must represent predicted values from machine learning models. & Representation of machine learning and predicted properties implies completeness and coverage. & Completeness, Coverage, Availability \\
\hline
REQ9: The ontology should be modular enough for diverse projects beyond its primary application. & Modularity and the ability to be used in diverse projects imply adaptability. & Adaptability, Modularity, Availability \\
\hline
\end{tabular}
\label{table:requirements}
\end{table}

McDaniel et al. \cite{Evaluating_domain_s_classification} categorized ontology evaluation into five distinct classes based on their cluster analysis findings. These classes include (1) error checking and ontology cleaning; (2) creating domain-specific libraries for ontology management; (3) utilizing metrics for quantifying ontology quality; (4) modularizing ontologies for assessment tasks; and (5) determining ontology fitness for specific tasks. In this work, we focus on metrics-based and error-checking evaluations as they are important for assessing ontology quality. These criteria allow us to quantitatively measure various aspects of the ontology's structure and identify potential errors or inconsistencies.


The ROBOT tool\footnote{\url{http://robot.obolibrary.org/}} \cite{jackson2019robot} and OntoMetrics \footnote{\url{https://ontometrics.informatik.uni-rostock.de/ontologymetrics/}} \cite{lantow2016ontometrics} were used to evaluate the ontologies and compute the ontological metrics. In this study, the metrics used for ontology evaluation are based on the ontology files as they were published, without applying reasoning. This means that the evaluation was conducted solely on the explicit information available in the ontologies. Metric-based approaches for ontology evaluation provide a perspective on the quantity of ontology elements \cite{Tartir2010_ontometrics}. These methods analyze the ontology to collect various statistical measures regarding the knowledge it contains. In the current study, axiom count, class count, object properties count, data property count, annotation assertions axiom count, and Description Logics (DL) expressivity have been used. In addition to the base metrics, schema metrics focus on the structure and design of the ontology, aiming to evaluate its potential for comprehensive knowledge representation \cite{Gangemi2006ModellingOE}. For schema metrics \cite{Tartir2010_ontometrics}, the attribute richness, inheritance richness, relationship richness, axiom/class ratio, and equivalence ratio have been analyzed. Attribute Richness (AR) \cite{Tartir2010_ontometrics} is a metric that represents the average number of attributes per class in ontology. Inheritance Richness (IR) \cite{Tartir2010_ontometrics} refers to the mean number of subclasses per class. Relationship Richness (RR) \cite{Tartir2010_ontometrics} is the fraction of non-inheritance relationships to the total number of relationships within the ontology. The Axiom Class Ratio \cite{lantow2016ontometrics} is determined by computing the mean number of axioms associated with each class in the ontology. Equivalence Ratio \cite{lantow2016ontometrics} is the ratio of equivalent classes to the total number of classes in ontology. These criteria are considered relevant for Materials Science and Engineering experts as it allows them to quantitatively assess the ontology's complexity, expressiveness, and logical relationships, providing valuable insights into the representation and quality of domain-specific knowledge.


For error-checking evaluations, the OOPS! (Ontology Pitfall Scanner!) tool \cite{poveda2014oops} was used to check the potential errors in the ontologies.

\input{sections/general-list}


==> sections/results_discussion_0.tex <==
\section{Results and Discussion}
\label{sec:results_discussion}


\subsection{Analysis of the MSE ontologies}
\label{sec:ontologies_results_section}

A total of 75 ontologies have been identified which can be found in \footnote{\href{https://docs.google.com/spreadsheets/d/1I4Ye2lrAn68mrd9edq1m6CYx2DdWgDFx/edit?usp=sharing&ouid=100247787073779135889&rtpof=true&sd=true}{Link to the list of ontologies}}. In this study, we evaluate 41 of these ontologies, which are MSE domain-specific. Table~\ref{tab:general-list} provides a comparison of these ontologies based on some general aspects. The MSE ontologies encompass various sub-domains, including Materials Characterization (including CHAMEO \cite{CHAMEO}, CIF-core, DISO \cite{diso_ontology}, and EMMO Crystallography ontologies), Nanomaterials (including NPO\cite{npo_ontology}, NanoMine \cite{nanomine_ontology}, and eNanoMapper \cite{enanomapper} ontologies), Mechanical Testing (including EMMO mechanical testing, MOL BRINELL, and MOL TENSILE ontologies), Process Modeling (including GPO, PMDCO \cite{pmdco}, and SMART-Protocols \cite{sp_ontology} ontologies) and Additive Manufacturing (including AMONTOLOGY and LPBFO \cite{lpbf_ontology} ontologies) and Batteries (including EMMO BattINFO and EMMO BVC ontologies). Each sub-domain is represented by two or more ontologies. Within the MSE ontologies, it was noted that EMMO is re-used in 12 ontologies, BWMD-MID in 3 ontologies, NPO in 2 ontologies, and SSN and GPO in 1 ontology each. EMMO, BFO \cite{bfo} and DOLCE \cite{dolce} are the top-level ontologies that are used in the list of MSE ontologies. \textit{Competency questions} specifying the requirements of the ontology are required to identify the types of possible queries users may want to make to a knowledge base based on an ontology \cite{uschold_gruninger_1996_competency}. However, only 5 of the investigated 41 MSE ontologies published their competency questions, which are DISO, MDO, PMDCO, OEO, and SMART-Protocols. Regarding the reuse of ontological resources, the adoption of Ontology Design Patterns (ODPs) as small and modular solutions to recurrent modeling problems \cite{Gangemi2009_odps} is rarely observed. The Stimulus-Sensor-Observation ODP \cite{sso_odp} is used in the SSN ontology and Provenance ODP \footnote{\url{http://ontologydesignpatterns.org/wiki/Submissions:Provenance}} is used in the MDO ontology. 


\subsection{Evaluation of the MSE ontologies}
\label{sec:evaluation_results_section}

Table~\ref{tab:base-metrics} presents structural measures for the MSE  ontologies. Axioms as the main components of an ontology state the truth within the domain. The axiom count is the total number of axioms present in the ontology. It provides a measure of the complexity and size of the ontology. NPO, MOL BRINELL, SEMMD, and OEO have higher axiom count compared to the other ontologies and likely provide a more complex and comprehensive representation of the domain's knowledge. A higher class count can also indicate increased complexity in the ontology. NPO, OEO, EMMO, VIMMP, and GPO have higher class counts which means that they have a larger number of distinct classes in the domain. The higher object property count indicates the complexity of relationships between entities. VIMMP, OEO, SEMMD, EMMO, and GPO have higher object property counts compared to the other ontologies. The data property count indicates the various attributes of individuals of classes in the ontology. Therefore, a higher data property count suggests a greater diversity of attributes being captured and represented in the ontology. VIMMP, DEB, MAMBO, SEMMD, and MDO have higher data property counts respectively. The number of classes and properties in an ontology is not necessarily an indicator of its use or relevance. It is essential to consider that many ontologies may contain a large number of classes and properties that are either not used at all or used very rarely in actual applications. Annotation assertions axioms are used to add additional information to entities in the ontology and indicate the extent of documentation and human-readable information provided in the ontology. NPO, OEO, SEMMD, EMMO, and GPO have higher annotation assertions axioms counts compared to the other ontologies.
%DL expressivity measures the expressive power of the ontology's logical language. Higher expressivity may allow more complex modeling but can also lead to increased computational complexity in reasoning tasks. SROIQ (D) Description Logic, which provides the expressiveness of OWL 2, is mostly used in the MSE ontologies. 

Table~\ref{tab:schema_metrics} provides the schema metrics evaluation for the MSE  ontologies. The greater the number of Attribute Richness (AR), the more detailed the description of entities in the domain, leading to a more expressive and comprehensive ontology. MAMBO, Periodictable, MDO, EMMO Datamodel, and SSOS show higher AR values. Among the MSE ontologies, Periodictable, EMMO Datamodel, GPO, AMONTOLOGY, and EMMO crystallography have the highest Inheritance Richness values which indicate that they are horizontal ontologies with numerous direct subclasses that contain a broad representation of general knowledge with less granularity. However, BMO, MAMBO, MOL BRINELL, MVC, and SSN have the lowest Inheritance Richness values among other ontologies which indicate that they are vertical ontologies with fewer direct subclasses that have a deep and specific domain coverage.

Ontologies SSN, NPO, MVC, BMO, and MAMBO have the highest Relationship Richness values among other ontologies which indicate a diverse range of relationships, leading to a richer representation of knowledge. A higher Axiom Class Ratio indicates a more complex and expressive representation between classes. The EquivalentClasses axiom states that multiple class expressions have the same meaning or refer to the same group of individuals, meaning that they contain identical sets of individuals \cite{hitzler2009owl}. Periodictable, MatOnto, MVC, NPO, VIMMP, PMDCO ontologies have the highest Equivalence Ratio, leading to less complexity, and improved interoperability and data integration across different systems or ontologies.

\input{sections/base-metrics}

\input{sections/schema_metrics}

\input{sections/graph-metrics}

Table \ref{tab:evaluation_oops} shows the results of ontology evaluation using the OOPS! tool \cite{poveda2014oops}. The pitfalls are categorized based on their importance level into Critical, Important, and Minor. The number in front of each pitfall indicates the number of ontology elements that are affected by the pitfall. Each pitfall is a potential error in ontology and the catalogue of pitfalls is available here\footnote{\url{https://oops.linkeddata.es/catalogue.jsp}}. Critical pitfalls impact ontology consistency, reasoning, and applicability. The results reveal the most repeated critical pitfalls as follows: P19 (Multiple domains or ranges defined for properties), leading to misinterpretation as a conjunction in OWL. P40 (Namespace hijacking), where terms from another namespace are used without proper definition, preventing information retrieval. P31, incorrect use of owl:equivalentClass for defining non-equivalent classes. P05, incorrect use of owl:inverseOf for defining non-inverse relationships. P29, incorrect use of owl:TransitiveProperty for defining non-transitive relationships. And P27 related to incorrect use of owl:equivalentProperty for defining non-equivalent properties. Important pitfalls, while not critical for ontology function, should still be addressed to ensure overall ontology quality. On the other hand, minor pitfalls, though not problematic, can be corrected to enhance ontology organization and user-friendliness \cite{poveda2014oops}.

\input{sections/evaluation_oops}

%\begin{figure}[H]
%\centering
%\includegraphics[width=\textwidth]{imgs/projects.png}
%\caption{projects.}
%\label{fig:projects}
%\end{figure}


%\begin{figure}[H]
%\centering
%\includegraphics[width=\textwidth]{imgs/n_citation.png}
%\caption{Number of citations.}
%\label{fig:n_citation}
%\end{figure}

